Scaling betweenness centrality using communication-efficient sparse matrix multiplication

Betweenness centrality (BC) is a crucial graph problem that measures the significance of a vertex by the number of shortest paths leading through it. We propose Maximal Frontier Betweenness Centrality (MFBC): a succinct BC algorithm based on novel sparse matrix multiplication routines that performs a factor of $p^{1/3}$ less communication on $p$ processors than the best known alternatives, for graphs with $n$ vertices and average degree $k=n/p^{2/3}$. We formulate, implement, and prove the correctness of MFBC for weighted graphs by leveraging monoids instead of semirings, which enables a surprisingly succinct formulation. MFBC scales well for both extremely sparse and relatively dense graphs. It automatically searches a space of distributed data decompositions and sparse matrix multiplication algorithms for the most advantageous configuration. The MFBC implementation outperforms the well-known CombBLAS library by up to 8x and shows more robust performance. Our design methodology is readily extensible to other graph problems.

==> Makefile <==
DOCUMENT=paper
TR=techreport

FILES=*.tex *.bib Makefile

all: $(DOCUMENT).pdf

.PHONY: gnuplots
gnuplots: gnuplots/*.plot gnuplots/*.dat
	$(MAKE) -C gnuplots

$(DOCUMENT).pdf: $(FILES) 
	#if [ -d img ]; then make -C img; fi
	rm -f pdflatex.out
	pdflatex $(DOCUMENT).tex 2>&1 | tee pdflatex.out
	if grep -q '\\cite{' *.tex; then bibtex $(DOCUMENT); fi;
	pdflatex $(DOCUMENT).tex 2>&1 | tee pdflatex.out
	pdflatex $(DOCUMENT).tex 2>&1 | tee pdflatex.out
	#dvips $(DOCUMENT).dvi -o $(DOCUMENT).ps
	#ps2pdf14 -dPDFSETTINGS=/printer -dAutoFilterColorImages=false -dColorImageFilter=/FlateEncode $(DOCUMENT).ps

tr: $(TR).pdf

$(TR).pdf: $(FILES)
	#if [ -d img ]; then make -C img; fi
	rm -f pdflatex.out
	pdflatex $(TR).tex 2>&1 | tee pdflatex.out
	if grep -q '\\cite{' *.tex; then bibtex $(TR); fi;
	pdflatex $(TR).tex 2>&1 | tee pdflatex.out
	pdflatex $(TR).tex 2>&1 | tee pdflatex.out
	#dvips $(DOCUMENT).dvi -o $(DOCUMENT).ps
	#ps2pdf14 -dPDFSETTINGS=/printer -dAutoFilterColorImages=false -dColorImageFilter=/FlateEncode $(DOCUMENT).ps
	cp $(TR).pdf ../package_for_spcl_website/sf_sc_2014/tr

show: $(DOCUMENT).pdf
	evince $(DOCUMENT).pdf

force: 
	rm -f $(DOCUMENT).pdf
	make $(DOCUMENT).pdf

clean:
	rm -f *.aux *.out  *.log
	rm -f $(DOCUMENT).blg $(DOCUMENT).dvi $(DOCUMENT).vrb
	rm -f $(DOCUMENT).pdf $(DOCUMENT).toc $(DOCUMENT).lo[a,f,g,h,l,t]
	rm -f $(DOCUMENT).nav $(DOCUMENT).snm $(DOCUMENT).ps
	rm -f history.txt llncs.cls llncs.dem llncs.ind llncsdoc.sty sprmindx.sty subjidx.ind llncs.dvi llncs.doc llncsdoc.pdf readme.txt
	rm -f *.aux *.out $(TR).bbl *.log
	rm -f $(TR).blg $(TR).dvi $(TR).vrb
	rm -f $(TR).pdf $(TR).toc $(TR).lo[a,f,g,h,l,t]
	rm -f $(TR).nav $(TR).snm $(TR).ps
	#if [ -f plt/Makefile ]; then make -C plt clean; fi
	#if [ -d img ]; then make -C img clean; fi
	#if [ -d slides ]; then make -C img clean; fi
	#if [ -d ../img ]; then make -C ../img clean; fi



==> bgrnd.tex <==
We first introduce the notation and concepts that enable a unified description
of various BC algorithms.  The most important employed symbols are summarized
in Table~\ref{tab:symbols}.

\subsection{Basic Graph Notation}

We start by presenting the used graph notation.
We represent an undirected unweighted labeled graph $G$ as a tuple $(V,E)$; $V=1:n =\{1,\ldots, n\}$ is a set of vertices
and $E \subseteq V \times V$ is a set of edges; $|V|=n$ and $|E|=m$. 
We denote the set of possible weight values as $\mathbb{W}\subset \mathbb{R}\cup \{\infty\}$.
If $G$ is weighted, we have $G = (V,E,w)$ where $w: E \to \mathbb{W}$ is a weight function.
We denote the adjacency matrix of $G$ as $\wA$; $\wA(i,j)=w(i,j)$ if $(i,j)\in E$, otherwise $\wA(i,j)=\infty$. 

\begin{table}
\centering
\small
\sf
\begin{tabular}{@{}l|ll@{}}
\toprule
\multirow{6}{*}{\begin{turn}{90}\shortstack{{Graph}\\{structure}}\end{turn}} & $G$&a given graph, $G=(V,E)$; $V$ and $E$ are sets of vertices and edges;\\
                   & & if $G$ is weighted, then $G=(V,E,w)$ where $w : E \to \mathbb{W}$.\\
                   & $n,m$&numbers of vertices and edges in $G$; $n = |V|, m = |E|$.\\
                   & $\rho(v)$&degree of $v$; $\overline{\rho}$ and $\rwh{\rho}$ are the average and maximum degree in $G$.\\
                   & $d$& diameter of a given graph $G$.\\ 
                   & $A$& adjacency matrix of $G$.\\
                   \midrule
\multirow{6}{*}{\begin{turn}{90}\shortstack{General BC}\end{turn}} 
                   & $\lambda(v)$ & betweenness centrality of $v$.\\ 
                   & $\tau(s,t)$&shortest path distance between $s,t$.\\
                   & $\bar\sigma(s,t)$& number of shortest paths between $s,t$.\\
                   & $\sigma(s,t,v)$& number of shortest paths between $s,t$ leading via $v$.\\
                   & $\delta(s,v)$ &  dependency of $s$ on $v$; $\delta(s,v) = \sum_{t \in V} {\sigma(s,t,v)}/{\bar\sigma(s,t)}$.\\
                   & $\pi(s,v)$ & set of immediate predecessors of $v$ in the shortest paths from $s$ to $v$.\\
\bottomrule
\end{tabular}
\vspace{+0.5em}
\caption{Symbols used in the paper; $v,s,t \in V$ are vertices.}
\label{tab:symbols}
\vspace{-0.5em}
\end{table}

\subsection{Algebraic Structures}

Next, we provide a unified algebraic notation for expressing different BC algorithms.
Instead of semirings, which are common in algebraic
graph algorithms, we employ commutative \emph{monoids}.
Semirings permit multiplicative operators only on elements within the same set,
while our algorithms require operators on members of different sets.
We use monoids to define generalized matrix-vector 
and matrix-matrix multiplication operators.

A monoid $(S, \oplus)$ is a set closed under an associative binary operation
$\oplus$ with an identity element.
A commutative monoid $(S,\oplus)$ is a monoid where $\oplus$ is commutative, and
\begin{gather*}
\bigoplus_{i=j}^k s(i) = s(j)\oplus s(j+1)\oplus \cdots \oplus s(k)
\end{gather*}
for any $k\geq j$ with $s(i)\in S$ for each $i\in j:k$.
We denote the elementwise application of a monoid operator to a pair
of matrices as $A\oplus B$ for any $A,B\in S^{m\times n}$.

\subsection{Generalized Matrix Multiplication}
To define a suitable matrix multiplication primitive for our algorithms, we
permit different domains for the matrices and replace elementwise multiplication
with an arbitrary function that is a suitable map between the domains. 
Specifically, consider two input matrices $A\in D_A^{m\times k}$ and $B\in
D_B^{k\times n}$, a bivariate function $f : D_A\times D_B \to D_C$,
and a commutative monoid $(D_C,\oplus)$.
Then, we denote matrix multiplication (MM) as $C=\MM{\oplus}{f}{A}{B}$, where each element 
of the output matrix, $C \in D_C^{m \times n}$, is
$C(i,j)=\bigoplus_{k=1}^nf(A(i,k), B(k,j))$, $\forall i\in 1:m, j\in 1:n$.
This MM notation enables a unified description of the main steps of
MFBC.

\subsection{Algebraic Graph Algorithms}

Most graph algorithms can be expressed via matrix-vector or matrix-matrix products.  
As an introductory example, we consider BFS~\cite{Cormen:2001:IA:580470}.  BFS starts
at a root vertex $r$ and traverses all nodes connected to $r$ by one edge, then the set of nodes two edges away from $r$, etc.
BFS can be used to compute shortest paths in an unweighted graph, which we can represent by an adjacency matrix with elements $A_{ij}\in\{1,\infty\}$. 
In this case, BFS would visit each vertex $v$ and derive its distance $\tau(r,v)$ from the root vertex $r$.

Algebraically, BFS can be expressed as iterative multiplication of the sparse adjacency matrix $A$ with a sparse 
vector $x_i$ over the tropical semiring, with $i$ denoting the iteration number. 
The tropical semiring is a commutative monoid 
$(\mathbb{W}, \min)$ combined with the addition operator, which replace the monoid $(\mathbb{R},+)$ and multiplication operator that are usually used within the matrix-vector product.
The BFS algorithm would initialize ${x}_0^r = 0$ (an
initial distance to $r$ is $0$) and any other element of ${x}_0$ is $\infty$
(i.e., an initial distance to any other element is $\infty$).
Each BFS iteration computes $x_{i+1}=\MM{\min}{+}{x_i}{A}$,
then screens $x_{i+1}$ retaining only elements that were $\infty$ in all $x_j$ for $j<i$.
The sparsity of the vector is given by all entries which are not equal to $\infty$, the additive identity of the tropical semiring.
\subsection{Brandes' Algorithm}
\label{sec:bc-spmm}

BC derives the importance of a vertex $v$ based on the number of
shortest paths that pass through $v$. Let $\bar\sigma(s,t)$ be the number of shortest
paths between two vertices $s,t$, and let $\sigma(s,t,v)$ be the
number of such paths that pass through $v$, $\sigma(s,s,v)=\sigma(s,t,s)=\sigma(s,t,t)=0$. 
The centrality score of $v$ is defined as $\lambda(v) =
\sum_{s,t \in V} \frac{\sigma(s,t,v)}{\bar\sigma(s,t)}$.
Define the
dependency of a source vertex $s$ on $v$ as: $\delta(s,v) = \sum_{t \in V}
\frac{\sigma(s,t,v)}{\bar\sigma(s,t)}$. Then, $\lambda(v) = \sum_{s  \in
V} \delta(s,v)$ where $\delta(s,v)$ satisfies the recurrence:
$\delta(s,v) = \sum_{w\in \pi(s,w)} \frac{\bar\sigma(s,v)}{\bar\sigma(s,w)} (1 +
\delta(s,w))$; $\pi(s,w)$ is a list of immediate predecessors of $w$ in the
shortest paths from $s$ to $w$.
Brandes' scheme~\cite{brandes2001faster} uses this recurrence to compute $\lambda(v)$ in two parts. First,
multiple concurrent BFS traversals compute $\pi(s,v)$ and $\bar\sigma(s,v)$,
$\forall{s,v \in V}$, obtaining a predecessor tree over $G$. Second, the tree is traversed
backwards (from the highest to the lowest distance) to compute $\delta(s,v)$
and $\lambda(v)$ based on the equations above.

Brandes' algorithm has been a subject of many previous efficiency studies
~\cite{jin2010novel,yang2005parallel,Bader:2006:PAE:1156433.1157604,madduri2009faster,prountzos2013betweenness,Kulkarni:2007:OPR:1250734.1250759,green2013faster,tan2009parallel,DBLP:journals/corr/abs-0809-1906,cong2012optimizing,tan2011analysis,shi2011fast,yang2011fast}.
Some efforts considered distributed memory parallelization~\cite{edmonds2010space,Bernaschi2016}.
The only distributed memory BC implementation done using matrix primitives we are aware of exists in CombBLAS~\cite{bulucc2011combinatorial}.
To the best of our knowledge, we provide the first communication cost analysis of a BC algorithm,
and the first implementation leveraging 3D sparse matrix multiplication.
A mix of graph replication and blocking have been previously used for BC computation~\cite{Bernaschi2016}, but the communication complexity of the scheme was not analyzed.
Furthermore, previous parallel codes and algebraic BC formulations have been limited to unweighted graphs.

\subsection{Cyclops Tensor Framework (CTF)}
\label{sec:ctf}






==> repr_apx.tex <==


We describe our benchmarking methodology in Section~\ref{sec:exp}.
Here, we provide some more technical details to allow reproduction of our results on the Blue Waters machine or a similar architecture.
We make our anonymized code for betweenness centrality available in the repository \url{https://github.com/solomonik/graph_centrality}.
The repository also includes a modified CombBLAS benchmark that generates uniform random graphs.

\macb{Compilation}

We built CTF using the Intel compiler module v5.2.82 with an additional gcc v5.3.0 module loaded.
We built CombBLAS using purely the gcc v5.2.82 module.
These modules were the latest available at the start of April 2017.

We built CTF with flags '-fast' and -no-ipo' as well as weith profiling output on.
We built CombBLAS with the default optimization flags '-O2'. 
No changes were made to the contents of either software internally to the aforementioned versions (CTF v1.4.1, ComBBLAS v1.5.0).

\macb{Execution}

We provide our submission job generation scripts below.
In some cases, we rerun parts of scripts if they did not complete in the expected time.

\macb{Real-World graphs}
\begin{verbatim}
#!/bin/bash

snp=$1
nodes=$((2*$snp*$snp))
p=$((32*$nodes))

cat > real.script$nodes.sh <<EOF
#!/bin/bash
#PBS -l nodes=$nodes:ppn=32:xe
#PBS -l walltime=03:00:00
#PBS -N ctf_btwn_central
#PBS -e \$PBS_JOBID.err
#PBS -o \$PBS_JOBID.out
#PBS -W umask=0027

cd \$PBS_O_WORKDIR

for bsize in 128 512 2048 8192
do
  aprun -n $p ./betwcent ../graphs/patents     
      1 \$bsize >> patents.p$p.\$PBS_JOBID
  aprun -n $p ./betwcent ../graphs/livejournal 
      1 \$bsize >> livejournal.p$p.\$PBS_JOBID
  aprun -n $p ./betwcent ../graphs/orkut       
      1 \$bsize >> orkut.p$p.\$PBS_JOBID
 aprun -n $p ./betwcent ../graphs/friendster  
      1 \$bsize >> friendster.p$p.\$PBS_JOBID

  aprun -n $p ./test_btwn_central -prep 1 -test 0 
      -bsize \$bsize -mwht 1 -nbatches 1 -n 6009554  
      -f ../graphs/patents/patents.txt 
      >> patents.p$p.\$PBS_JOBID
  aprun -n $p ./test_btwn_central -prep 1 -test 0 
      -bsize \$bsize -mwht 1 -nbatches 1 -n 4847571  
      -f ../graphs/livejournal/livejournal.txt
      >> livejournal.p$p.\$PBS_JOBID
  aprun -n $p ./test_btwn_central -prep 1 -test 0 
      -bsize \$bsize -mwht 1 -nbatches 1 -n 3072441  
      -f ../graphs/orkut/orkut.txt 
      >> orkut.p$p.\$PBS_JOBID
  aprun -n $p ./test_btwn_central -prep 1 -test 0 
      -bsize \$bsize -mwht 1 -nbatches 1 -n 65608366 
      -f ../graphs/friendster/friendster.txt 
      >> friendster.p$p.\$PBS_JOBID
done
EOF
\end{verbatim}

\macb{R-MAT graphs}

\begin{verbatim}
#!/bin/bash

snp=$1
nodes=$((2*$snp*$snp))
p=$((32*$nodes))
sqrt_p=$((8*$snp))
cat > rmat.script$nodes.sh <<EOF
#!/bin/bash
#PBS -l nodes=$nodes:ppn=32:xe
#PBS -l walltime=02:00:00
#PBS -N ctf_btwn_central
#PBS -e \$PBS_JOBID.err
#PBS -o \$PBS_JOBID.out
#PBS -W umask=0027

cd \$PBS_O_WORKDIR

for bsize in 128 512 2048 8192
do
  aprun -n $p ./betwcent ../graphs/rmat_e8  1 \$bsize 
      >> rmat.S22.E8.p$p.\$PBS_JOBID
  aprun -n $p ./test_btwn_central -prep 1 -test 0 
      -bsize \$bsize -mwht 1 -nbatches 1 -S 22 -E 8 
      >> rmat.S22.E8.p$p.\$PBS_JOBID
  aprun -n $p ./test_btwn_central -prep 1 -test 0 
      -bsize \$bsize -mwht 1 -nbatches 1 -S 22 -E 8 
      -adapt 0 >> rmat.S22.E8.p$p.\$PBS_JOBID
  aprun -n $p ./test_btwn_central -prep 1 -test 0 
      -bsize \$bsize -mwht 1 -nbatches 1 -S 22 -E 8 
      -adapt 0 -sp_C 0 >> rmat.S22.E8.p$p.\$PBS_JOBID
  aprun -n $p ./test_btwn_central -prep 1 -test 0 
      -bsize \$bsize -mwht 1 -nbatches 1 -S 22 -E 8 
      -adapt 0 -sp_C 0 -sp_B 0 
      >> rmat.S22.E8.p$p.\$PBS_JOBID
  aprun -n $p ./test_btwn_central -prep 1 -test 0 
      -bsize \$bsize -mwht 100 -nbatches 1 -S 22 -E 8 
      >> rmat.S22.E8.p$p.\$PBS_JOBID

  aprun -n $p ./betwcent ../graphs/rmat_e128  1 
      \$bsize >> rmat.S22.E128.p$p.\$PBS_JOBID
  aprun -n $p ./test_btwn_central -prep 1 -test 0 
      -bsize \$bsize -mwht 1 -nbatches 1 -S 22 -E 128 
      >> rmat.S22.E128.p$p.\$PBS_JOBID
  aprun -n $p ./test_btwn_central -prep 1 -test 0 
      -bsize \$bsize -mwht 1 -nbatches 1 -S 22 -E 128 
      -adapt 0 >> rmat.S22.E128.p$p.\$PBS_JOBID
  aprun -n $p ./test_btwn_central -prep 1 -test 0 
      -bsize \$bsize -mwht 1 -nbatches 1 -S 22 -E 128 
      -adapt 0 -sp_C 0 >> rmat.S22.E128.p$p.\$PBS_JOBID
  aprun -n $p ./test_btwn_central -prep 1 -test 0 
      -bsize \$bsize -mwht 1 -nbatches 1 -S 22 -E 128 
      -adapt 0 -sp_C 0 -sp_B 0 
      >> rmat.S22.E128.p$p.\$PBS_JOBID
  aprun -n $p ./test_btwn_central -prep 1 -test 0 
      -bsize \$bsize -mwht 100 -nbatches 1 -S 22 -E 128 
      >> rmat.S22.E128.p$p.\$PBS_JOBID
done
EOF\end{verbatim}
\macb{Random-uniform graphs}

\begin{verbatim}
#!/bin/bash

snp=$1
nodes=$((2*$snp*$snp))
p=$((32*$nodes))
sqrt_p=$((8*$snp))
n0=131072
n1=1310720
n0_escl=$(($n0*$snp))
n0_vscl=$(($n0*$snp*$snp))
n1_escl=$(($n1*$snp))
n1_vscl=$(($n1*$snp*$snp))
f_nnz00=.005
f_nnz01=.0001
f_nnz10=.0005
f_nnz11=.00001
f_vscl_nnz00=$(echo "$f_nnz00/($snp*$snp)" | bc -l)
f_vscl_nnz01=$(echo "$f_nnz01/($snp*$snp)" | bc -l)
f_vscl_nnz10=$(echo "$f_nnz10/($snp*$snp)" | bc -l)
f_vscl_nnz11=$(echo "$f_nnz11/($snp*$snp)" | bc -l)

cat > unif.script$nodes.sh <<EOF
#!/bin/bash
#PBS -l nodes=$nodes:ppn=32:xe
#PBS -l walltime=02:00:00
#PBS -N ctf_btwn_central
#PBS -e \$PBS_JOBID.err
#PBS -o \$PBS_JOBID.out
#PBS -W umask=0027

cd \$PBS_O_WORKDIR

for bsize in 128 512 2048 8192
do
  aprun -n $p ./betwcent_unif $n0_escl $f_nnz00 1 \$bsize 
    >> unif.n$n0_escl.sp$f_nnz00.p$p.\$PBS_JOBID
  aprun -n $p ./betwcent_unif $n0_escl $f_nnz01 1 \$bsize 
    >> unif.n$n0_escl.sp$f_nnz01.p$p.\$PBS_JOBID
  aprun -n $p ./betwcent_unif $n1_escl $f_nnz10 1 \$bsize 
    >> unif.n$n1_escl.sp$f_nnz10.p$p.\$PBS_JOBID
  aprun -n $p ./betwcent_unif $n1_escl $f_nnz11 1 \$bsize 
    >> unif.n$n1_escl.sp$f_nnz11.p$p.\$PBS_JOBID

  aprun -n $p ./test_btwn_central -prep 1 -test 0 -bsize \$bsize 
    -mwht 1 -nbatches 1 -n $n0_escl -sp $f_nnz00 
    >> unif.n$n0_escl.sp$f_nnz00.p$p.\$PBS_JOBID
  aprun -n $p ./test_btwn_central -prep 1 -test 0 -bsize \$bsize 
    -mwht 1 -nbatches 1 -n $n0_escl -sp $f_nnz01
    >> unif.n$n0_escl.sp$f_nnz01.p$p.\$PBS_JOBID
  aprun -n $p ./test_btwn_central -prep 1 -test 0 -bsize \$bsize 
    -mwht 1 -nbatches 1 -n $n1_escl -sp $f_nnz10 
    >> unif.n$n1_escl.sp$f_nnz10.p$p.\$PBS_JOBID
  aprun -n $p ./test_btwn_central -prep 1 -test 0 -bsize \$bsize 
    -mwht 1 -nbatches 1 -n $n1_escl -sp $f_nnz11 
    >> unif.n$n1_escl.sp$f_nnz11.p$p.\$PBS_JOBID

  aprun -n $p ./betwcent_unif $n0_vscl $f_vscl_nnz00 1 
    \$bsize >> unif.n$n0_vscl.sp0.p$p.\$PBS_JOBID
  aprun -n $p ./betwcent_unif $n0_vscl $f_vscl_nnz01 1 
    \$bsize >> unif.n$n0_vscl.sp1.p$p.\$PBS_JOBID
  aprun -n $p ./betwcent_unif $n1_vscl $f_vscl_nnz10 1 
    \$bsize >> unif.n$n1_vscl.sp0.p$p.\$PBS_JOBID
  aprun -n $p ./betwcent_unif $n1_vscl $f_vscl_nnz11 1 
    \$bsize >> unif.n$n1_vscl.sp1.p$p.\$PBS_JOBID

  aprun -n $p ./test_btwn_central -prep 1 -test 0 -bsize \$bsize 
    -mwht 1 -nbatches 1 -n $n0_vscl 
    -sp $f_vscl_nnz00 >> unif.n$n0_vscl.sp0.p$p.\$PBS_JOBID
  aprun -n $p ./test_btwn_central -prep 1 -test 0 -bsize \$bsize 
    -mwht 1 -nbatches 1 -n $n0_vscl -sp $f_vscl_nnz01 
    >> unif.n$n0_vscl.sp1.p$p.\$PBS_JOBID
  aprun -n $p ./test_btwn_central -prep 1 -test 0 -bsize \$bsize 
    -mwht 1 -nbatches 1 -n $n1_vscl -sp $f_vscl_nnz10 
    >> unif.n$n1_vscl.sp0.p$p.\$PBS_JOBID
  aprun -n $p ./test_btwn_central -prep 1 -test 0 -bsize \$bsize 
    -mwht 1 -nbatches 1 -n $n1_vscl -sp $f_vscl_nnz11 
    >> unif.n$n1_vscl.sp1.p$p.\$PBS_JOBID
done
EOF
\end{verbatim}

